High-Order Deep Meta-Learning with Category-Theoretic Interpretation

We introduce a new hierarchical deep learning framework for recursive higher-order meta-learning that enables neural networks (NNs) to construct, solve, and generalise across hierarchies of tasks. Central to this approach is a generative mechanism that creates \emph{virtual tasks} -- synthetic problem instances designed to enable the meta-learner to learn \emph{soft constraints} and unknown generalisable rules across related tasks. Crucially, this enables the framework to generate its own informative, task-grounded datasets thereby freeing machine learning (ML) training from the limitations of relying entirely on human-generated data. By actively exploring the virtual point landscape and seeking out tasks lower-level learners find difficult, the meta-learner iteratively refines constraint regions. This enhances inductive biases, regularises the adaptation process, and produces novel, unanticipated tasks and constraints required for generalisation. Each meta-level of the hierarchy corresponds to a progressively abstracted generalisation of problems solved at lower levels, enabling a structured and interpretable learning progression. By interpreting meta-learners as category-theoretic \emph{functors} that generate and condition a hierarchy of subordinate learners, we establish a compositional structure that supports abstraction and knowledge transfer across progressively generalised tasks. The category-theoretic perspective unifies existing meta-learning models and reveals how learning processes can be transformed and compared through functorial relationships, while offering practical design principles for structuring meta-learning. We speculate this architecture may underpin the next generation of NNs capable of autonomously generating novel, instructive tasks and their solutions, thereby advancing ML towards general artificial intelligence.

==> mathdef.tex <==


% \DeclareMathOperator*{\E}{\mathbb{E}}
% \DeclareMathOperator*{\argmax}{argmax}
% \DeclareMathOperator*{\argmin}{argmin}
\newcommand{\Log}{\log \ }

\renewcommand{\S}{\mathbb{S}} 
% \newcommand{\R}{\mathbb{R}} 
\newcommand{\Rnn}{\mathbb{R}_{\ge 0}} 
% \newcommand{\Var}{\text{Var}}
\newcommand{\bfone}{\bm{1}}
\newcommand{\IQC}{\bm{IQC}}
% \newcommand{\U}{\mathbb{U}} 
\renewcommand{\P}{\mathbb{P}} 

% \newcommand{\E}{\mathbb{E}}
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cP}{{\mathcal P}} 
\newcommand{\cQ}{{\mathcal Q}} 
\newcommand{\cR}{{\mathcal R}} 
\newcommand{\cS}{{\mathcal S}} 
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cZ}{{\mathcal Z}}

\newcommand{\bma}{{\bm a}}
\newcommand{\bmb}{{\bm b}}
\newcommand{\bmc}{{\bm c}}
\newcommand{\bmd}{{\bm d}}
\newcommand{\bme}{{\bm e}}
\newcommand{\bmf}{{\bm f}}
\newcommand{\bmg}{{\bm g}}
\newcommand{\bmh}{{\bm h}}
\newcommand{\bml}{{\bm l}}
\newcommand{\bmm}{{\bm m}}
\newcommand{\bmk}{{\bm k}}
\newcommand{\bmo}{{\bm o}}
\newcommand{\bmp}{{\bm p}}
\newcommand{\bmr}{{\bm r}}
\newcommand{\bms}{{\bm s}}
\newcommand{\bmt}{{\bm t}}
\newcommand{\bmq}{{\bm q}}
\newcommand{\bmu}{{\bm u}}
\newcommand{\bmv}{{\bm v}}
\newcommand{\bmw}{{\bm w}}

\newcommand{\bmx}{{\bm x}}
\newcommand{\bmy}{{\bm y}}
\newcommand{\bmz}{{\bm z}}

\newcommand{\bmA}{{\bm A}}
\newcommand{\bmB}{{\bm B}}
\newcommand{\bmC}{{\bm C}}
\newcommand{\bmD}{{\bm D}}
\newcommand{\bmE}{{\bm E}}
\newcommand{\bmF}{{\bm F}}
\newcommand{\bmG}{{\bm G}}
\newcommand{\bmI}{{\bm I}}
\newcommand{\bmJ}{{\bm J}}
\newcommand{\bmH}{{\bm H}}
\newcommand{\bmK}{{\bm K}}
\newcommand{\bmL}{{\bm L}}
\newcommand{\bmM}{{\bm M}}
\newcommand{\bmN}{{\bm N}}
\newcommand{\bmP}{{\bm P}}
\newcommand{\bmQ}{{\bm Q}}
\newcommand{\bmR}{{\bm R}}
\newcommand{\bmS}{{\bm S}}
\newcommand{\bmT}{{\bm T}}
\newcommand{\bmV}{{\bm V}}
\newcommand{\bmU}{{\bm U}}
\newcommand{\bmW}{{\bm W}}
\newcommand{\bmX}{{\bm X}}
\newcommand{\bmY}{{\bm Y}}
\newcommand{\bmZ}{{\bm Z}}


\newcommand{\bmalpha}{{\bm \alpha}}
\newcommand{\bmbeta}{{\bm \beta}}
\newcommand{\bmdelta}{{\bm \delta}}
\newcommand{\bmeta}{{\bm \eta}}
\newcommand{\bmmu}{{\bm \mu}}
\newcommand{\bmnu}{{\bm \nu}}
\newcommand{\bmkappa}{{\bm \kappa}}
\newcommand{\bmpsi}{{\bm \psi}}
\newcommand{\bmphi}{{\bm \phi}}
\newcommand{\bmxi}{{\bm \xi}}
\newcommand{\bmlambda}{{\bm \lambda}}
\newcommand{\bmsigma}{{\bm \sigma}}
\newcommand{\bmrho}{{\bm \rho}}
\newcommand{\bmtheta}{{\bm \theta}}
\newcommand{\bmzeta}{{\bm \zeta}}

\newcommand{\bmSigma}{{\bm \Sigma}}
\newcommand{\bmOmega}{{\bm \Omega}}
\newcommand{\bmLambda}{{\bm \Lambda}}
\newcommand{\bmGamma}{{\bm \Gamma}}
\newcommand{\bmDelta}{{\bm \Delta}}
\newcommand{\bmPsi}{{\bm \Psi}}

\newcommand{\svec}[1]{\textrm{vec}\left(#1\right)}
\newcommand{\svecinv}[1]{\textrm{vec}^{-1}\left(#1\right)}
\newcommand{\smat}[1]{\textrm{mat}\left(#1\right)}
\newcommand{\transpose}{\textrm{T}}
\newcommand{\htranspose}{\textrm{H}}
\newcommand{\trace}[1]{\textrm{trace}\left(#1\right)} 
\newcommand{\rank}[1]{\textrm{rank}\left(#1\right)} 
\newcommand{\diag}[1]{{\rm diag}\left\{#1\right\}}
\newcommand{\blkdiag}[1]{{\rm blkdiag}\left\{#1\right\}}
\newcommand{\bmone}{{\bm 1}}
\newcommand{\bmzero}{{\bm 0}}
\newcommand{\conv}[1]{\textrm{conv}\left\{#1\right\}}
\newcommand{\circul}[1]{\textrm{circ}\left(#1\right)}
\newcommand{\doubcirc}[1]{\textrm{circ}^2\left(#1\right)}
\newcommand{\pad}[1]{\textrm{pad}\left(#1\right)}
\newcommand{\SDD}{\mathcal{SDD}}
\newcommand{\DD}{\mathcal{DD}}
\newcommand{\cFW}{\mathcal{FW}}
\newcommand{\cN}{\mathcal N}
\newcommand{\Dir}{\textrm{Dir}}
% \newcommand{\Beta}{\textrm{Beta}}
\newcommand{\Beta}{\mathbf{Beta}}
% \newcommand{\DP}{\textrm{DP}}
\newcommand{\DP}{\mathbf{DP}}
\newcommand{\Cat}{\mathbf{Cat}}
\newcommand{\Mul}{\textrm{Mul}}
\newcommand{\GEM}{\textrm{GEM}}
\newcommand{\ELBO}{\textrm{ELBO}}
\newcommand{\MLP}{\textrm{MLP}}
\newcommand{\Ber}{\textrm{Bernoulli}}
% \newcommand{\exp}{\textrm{exp}}
% \newcommand{\KL}[2]{{\cal KL}\left(#1 \,||\, #2\right)}


% \newtheorem{example}{Example}
% \newtheorem{prop}{Proposition}
% \newtheorem{rem}{Remark}
% \newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{asm}{Assumption}
\newtheorem{defn}{Definition}
% \newenvironment{proof}{\paragraph{Proof:}}{\hfill$\square$}
\newenvironment{proof_of}[1]{\paragraph{Proof of #1:}}{\hfill$\square$}


